Can LLM Watermarks Robustly Prevent Unauthorized Knowledge Distillation?

The radioactive nature of Large Language Model (LLM) watermarking enables the detection of watermarks inherited by student models when trained on the outputs of watermarked teacher models, making it a promising tool for preventing unauthorized knowledge distillation. However, the robustness of watermark radioactivity against adversarial actors remains largely unexplored. In this paper, we investigate whether student models can acquire the capabilities of teacher models through knowledge distillation while avoiding watermark inheritance. We propose two categories of watermark removal approaches: pre-distillation removal through untargeted and targeted training data paraphrasing (UP and TP), and post-distillation removal through inference-time watermark neutralization (WN). Extensive experiments across multiple model pairs, watermarking schemes and hyper-parameter settings demonstrate that both TP and WN thoroughly eliminate inherited watermarks, with WN achieving this while maintaining knowledge transfer efficiency and low computational overhead. Given the ongoing deployment of watermarking techniques in production LLMs, these findings emphasize the urgent need for more robust defense strategies. Our code is available at https://github.com/THU-BPM/Watermark-Radioactivity-Attack.

==> table/knowledge_gemma.tex <==
\begin{table*}[h!]
    \caption{Knowledge-Gemma}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        \textbf{Benchmark} &
        \textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
        \midrule
        \multirow{6}{*}{\makecell{ARC \\ Challenge \\ (ACC)}} & \multirow{6}{*}{0.4036} & \multirow{3}{*}{KGW} & $n=1$ & 0.4180 & 0.4100 \textcolor[rgb]{0.5,0.0,0.0}{(-1.9\%)} & 0.3980 \textcolor[rgb]{0.5,0.0,0.0}{(-4.8\%)} & \underline{\textbf{0.4210}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.7\%)} \\
        & & & $n=2$ & 0.4300 & 0.4010 \textcolor[rgb]{0.5,0.0,0.0}{(-6.7\%)} & 0.3850 \textcolor[rgb]{0.5,0.0,0.0}{(-10.5\%)} & \underline{\textbf{0.4320}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
        & & & $n=3$ & 0.4420 & 0.4090 \textcolor[rgb]{0.5,0.0,0.0}{(-7.5\%)} & 0.3920 \textcolor[rgb]{0.5,0.0,0.0}{(-11.3\%)} & \underline{\textbf{0.4440}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.4160 & 0.3880 \textcolor[rgb]{0.5,0.0,0.0}{(-6.7\%)} & 0.3800 \textcolor[rgb]{0.5,0.0,0.0}{(-8.7\%)} & \underline{\textbf{0.4190}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.7\%)} \\
        & & & $n=2$ & 0.4280 & 0.4080 \textcolor[rgb]{0.5,0.0,0.0}{(-4.7\%)} & 0.3950 \textcolor[rgb]{0.5,0.0,0.0}{(-7.7\%)} & \underline{\textbf{0.4300}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
        & & & $n=3$ & 0.4380 & 0.4120 \textcolor[rgb]{0.5,0.0,0.0}{(-6.0\%)} & 0.4000 \textcolor[rgb]{0.5,0.0,0.0}{(-8.7\%)} & \underline{\textbf{0.4400}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\

        \midrule
        \multirow{6}{*}{\makecell{TruthfulQA \\ Multiple Choice \\ (ACC)}} & \multirow{6}{*}{0.3311} & \multirow{3}{*}{KGW} & $n=1$ & 0.3450 & 0.3360 \textcolor[rgb]{0.5,0.0,0.0}{(-2.6\%)} & 0.3300 \textcolor[rgb]{0.5,0.0,0.0}{(-4.3\%)} & \underline{\textbf{0.3480}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.9\%)} \\
        & & & $n=2$ & 0.3580 & 0.3360 \textcolor[rgb]{0.5,0.0,0.0}{(-6.1\%)} & 0.3250 \textcolor[rgb]{0.5,0.0,0.0}{(-9.2\%)} & \underline{\textbf{0.3600}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=3$ & 0.3680 & 0.3480 \textcolor[rgb]{0.5,0.0,0.0}{(-5.4\%)} & 0.3330 \textcolor[rgb]{0.5,0.0,0.0}{(-9.5\%)} & \underline{\textbf{0.3700}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.3420 & 0.3250 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} & 0.3150 \textcolor[rgb]{0.5,0.0,0.0}{(-7.9\%)} & \underline{\textbf{0.3440}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=2$ & 0.3550 & 0.3380 \textcolor[rgb]{0.5,0.0,0.0}{(-4.6\%)} & 0.3280 \textcolor[rgb]{0.5,0.0,0.0}{(-7.5\%)} & \underline{\textbf{0.3570}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=3$ & \underline{\textbf{0.3650}} & 0.3450 \textcolor[rgb]{0.5,0.0,0.0}{(-5.5\%)} & 0.3330 \textcolor[rgb]{0.5,0.0,0.0}{(-8.8\%)} & 0.3630 \textcolor[rgb]{0.5,0.0,0.0}{(-0.5\%)} \\
        
        \midrule
        \multirow{6}{*}{\makecell{MTBench \\ (Full Score: 10)}} & \multirow{6}{*}{1.52} & \multirow{3}{*}{KGW} & $n=1$ & 1.65 & 1.48 \textcolor[rgb]{0.5,0.0,0.0}{(-10.3\%)} & 1.38 \textcolor[rgb]{0.5,0.0,0.0}{(-16.4\%)} & \underline{\textbf{1.66}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=2$ & 1.72 & 1.53 \textcolor[rgb]{0.5,0.0,0.0}{(-11.0\%)} & 1.41 \textcolor[rgb]{0.5,0.0,0.0}{(-18.0\%)} & \underline{\textbf{1.73}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=3$ & 1.78 & 1.57 \textcolor[rgb]{0.5,0.0,0.0}{(-11.8\%)} & 1.45 \textcolor[rgb]{0.5,0.0,0.0}{(-18.5\%)} & \underline{\textbf{1.79}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 1.67 & 1.50 \textcolor[rgb]{0.5,0.0,0.0}{(-10.2\%)} & 1.39 \textcolor[rgb]{0.5,0.0,0.0}{(-16.8\%)} & \underline{\textbf{1.68}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=2$ & 1.75 & 1.56 \textcolor[rgb]{0.5,0.0,0.0}{(-10.9\%)} & 1.44 \textcolor[rgb]{0.5,0.0,0.0}{(-17.7\%)} & \underline{\textbf{1.76}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=3$ & 1.82 & 1.61 \textcolor[rgb]{0.5,0.0,0.0}{(-11.5\%)} & 1.48 \textcolor[rgb]{0.5,0.0,0.0}{(-18.7\%)} & \underline{\textbf{1.83}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:knowledge_gemma}
\end{table*}

==> table/knowledge_llama38b_llama17b.tex <==
\begin{table*}[h!]
    \caption{Knowledge: Llama-3-8b-Instruct, Llama-7b}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        \textbf{Benchmark} &
        \textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
        \midrule
        \multirow{6}{*}{\makecell{ARC \\ Challenge \\ (ACC)}} 
        & \multirow{6}{*}{0.4181} 
        & \multirow{3}{*}{KGW} & $n=1$ & 0.4412 & 0.4138 \textcolor[rgb]{0.5,0.0,0.0}{(-6.2\%)} & 0.4005 \textcolor[rgb]{0.5,0.0,0.0}{(-9.2\%)} & 0.4373 \textcolor[rgb]{0.5,0.0,0.0}{(-0.9\%)} \\
        & & & $n=2$ & 0.4305 & 0.4180 \textcolor[rgb]{0.5,0.0,0.0}{(-2.9\%)} & 0.4022 \textcolor[rgb]{0.5,0.0,0.0}{(-6.6\%)} & \underline{\textbf{0.4389}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.9\%)} \\
        & & & $n=3$ & \underline{\textbf{0.4680}} & 0.3760 \textcolor[rgb]{0.5,0.0,0.0}{(-19.7\%)} & 0.3748 \textcolor[rgb]{0.5,0.0,0.0}{(-19.9\%)} & 0.4535 \textcolor[rgb]{0.5,0.0,0.0}{(-3.1\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.4375 & 0.4262 \textcolor[rgb]{0.5,0.0,0.0}{(-2.6\%)} & 0.4123 \textcolor[rgb]{0.5,0.0,0.0}{(-5.8\%)} & \underline{\textbf{0.4441}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.5\%)} \\
        & & & $n=2$ & 0.4238 & 0.4197 \textcolor[rgb]{0.5,0.0,0.0}{(-1.0\%)} & 0.4085 \textcolor[rgb]{0.5,0.0,0.0}{(-3.6\%)} & \underline{\textbf{0.4382}} \textcolor[rgb]{0.0,0.5,0.0}{(+3.4\%)} \\
        & & & $n=3$ & \underline{\textbf{0.4450}} & 0.4321 \textcolor[rgb]{0.5,0.0,0.0}{(-2.9\%)} & 0.4212 \textcolor[rgb]{0.5,0.0,0.0}{(-5.4\%)} & 0.4415 \textcolor[rgb]{0.5,0.0,0.0}{(-0.8\%)} \\
        
        \midrule
        \multirow{6}{*}{\makecell{TruthfulQA \\ Multiple Choice \\ (ACC)}} 
        & \multirow{6}{*}{0.3407} 
        & \multirow{3}{*}{KGW} & $n=1$ & 0.3825 & 0.3740 \textcolor[rgb]{0.5,0.0,0.0}{(-2.2\%)} & 0.3695 \textcolor[rgb]{0.5,0.0,0.0}{(-3.4\%)} & \underline{\textbf{0.4110}} \textcolor[rgb]{0.0,0.5,0.0}{(+7.4\%)} \\
        & & & $n=2$ & \underline{\textbf{0.4280}} & 0.3992 \textcolor[rgb]{0.5,0.0,0.0}{(-6.7\%)} & 0.3978 \textcolor[rgb]{0.5,0.0,0.0}{(-7.1\%)} & 0.4225 \textcolor[rgb]{0.5,0.0,0.0}{(-1.3\%)} \\
        & & & $n=3$ & 0.4360 & 0.4205 \textcolor[rgb]{0.5,0.0,0.0}{(-3.5\%)} & 0.3940 \textcolor[rgb]{0.5,0.0,0.0}{(-9.6\%)} & \underline{\textbf{0.4512}} \textcolor[rgb]{0.0,0.5,0.0}{(+3.5\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.3940 & 0.3845 \textcolor[rgb]{0.5,0.0,0.0}{(-2.4\%)} & 0.3750 \textcolor[rgb]{0.5,0.0,0.0}{(-4.8\%)} & \underline{\textbf{0.4135}} \textcolor[rgb]{0.0,0.5,0.0}{(+4.9\%)} \\
        & & & $n=2$ & 0.3860 & 0.3812 \textcolor[rgb]{0.5,0.0,0.0}{(-1.2\%)} & 0.3785 \textcolor[rgb]{0.5,0.0,0.0}{(-1.9\%)} & \underline{\textbf{0.4150}} \textcolor[rgb]{0.0,0.5,0.0}{(+7.5\%)} \\
        & & & $n=3$ & 0.3980 & 0.3885 \textcolor[rgb]{0.5,0.0,0.0}{(-2.4\%)} & 0.3920 \textcolor[rgb]{0.5,0.0,0.0}{(-1.5\%)} & \underline{\textbf{0.4205}} \textcolor[rgb]{0.0,0.5,0.0}{(+5.5\%)} \\
        
        \midrule
        \multirow{6}{*}{\makecell{MTBench \\ (Full Score: 10)}} 
        & \multirow{6}{*}{2.64} 
        & \multirow{3}{*}{KGW} & $n=1$ & 3.84 & 2.99 \textcolor[rgb]{0.5,0.0,0.0}{(-22.1\%)} & 2.69 \textcolor[rgb]{0.5,0.0,0.0}{(-30.0\%)} & \underline{\textbf{3.91}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.8\%)} \\
        & & & $n=2$ & \underline{\textbf{4.04}} & 3.34 \textcolor[rgb]{0.5,0.0,0.0}{(-17.3\%)} & 2.89 \textcolor[rgb]{0.5,0.0,0.0}{(-28.5\%)} & 3.97 \textcolor[rgb]{0.5,0.0,0.0}{(-1.7\%)} \\
        & & & $n=3$ & \underline{\textbf{4.17}} & 3.24 \textcolor[rgb]{0.5,0.0,0.0}{(-22.3\%)} & 2.99 \textcolor[rgb]{0.5,0.0,0.0}{(-28.3\%)} & 4.04 \textcolor[rgb]{0.5,0.0,0.0}{(-3.1\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & \underline{\textbf{4.09}} & 3.19 \textcolor[rgb]{0.5,0.0,0.0}{(-22.0\%)} & 2.04 \textcolor[rgb]{0.5,0.0,0.0}{(-50.1\%)} & 4.07 \textcolor[rgb]{0.5,0.0,0.0}{(-0.5\%)} \\
        & & & $n=2$ & \underline{\textbf{4.19}} & 2.99 \textcolor[rgb]{0.5,0.0,0.0}{(-28.6\%)} & 2.79 \textcolor[rgb]{0.5,0.0,0.0}{(-33.4\%)} & 4.14 \textcolor[rgb]{0.5,0.0,0.0}{(-1.2\%)} \\
        & & & $n=3$ & \underline{\textbf{4.21}} & 2.84 \textcolor[rgb]{0.5,0.0,0.0}{(-32.5\%)} & 2.64 \textcolor[rgb]{0.5,0.0,0.0}{(-37.3\%)} & 4.17 \textcolor[rgb]{0.5,0.0,0.0}{(-0.9\%)} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:knowledge_llama38b_llama17b}
\end{table*}

==> table/knowledge_llama38b_llama321b.tex <==
\begin{table*}[h!]
    \caption{Knowledge: Llama-3-8b-Instruct, Llama-3.2-1b}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        \textbf{Benchmark} &
        \textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
        \midrule
        \multirow{6}{*}{\makecell{ARC \\ Challenge \\ (ACC)}} 
        & \multirow{6}{*}{0.3166} 
        & \multirow{3}{*}{KGW} & $n=1$ & 0.3350 & 0.3198 \textcolor[rgb]{0.5,0.0,0.0}{(-4.5\%)} & 0.3025 \textcolor[rgb]{0.5,0.0,0.0}{(-9.7\%)} & \underline{\textbf{0.3452}} \textcolor[rgb]{0.0,0.5,0.0}{(+3.0\%)} \\
        & & & $n=2$ & \underline{\textbf{0.3460}} & 0.3175 \textcolor[rgb]{0.5,0.0,0.0}{(-8.2\%)} & 0.2810 \textcolor[rgb]{0.5,0.0,0.0}{(-18.8\%)} & 0.3418 \textcolor[rgb]{0.5,0.0,0.0}{(-1.2\%)} \\
        & & & $n=3$ & \underline{\textbf{0.3655}} & 0.3058 \textcolor[rgb]{0.5,0.0,0.0}{(-16.3\%)} & 0.2920 \textcolor[rgb]{0.5,0.0,0.0}{(-20.1\%)} & 0.3582 \textcolor[rgb]{0.5,0.0,0.0}{(-2.0\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.3482 & 0.3215 \textcolor[rgb]{0.5,0.0,0.0}{(-7.7\%)} & 0.3200 \textcolor[rgb]{0.5,0.0,0.0}{(-8.1\%)} & \underline{\textbf{0.3575}} \textcolor[rgb]{0.0,0.5,0.0}{(+2.7\%)} \\
        & & & $n=2$ & 0.3420 & 0.3301 \textcolor[rgb]{0.5,0.0,0.0}{(-3.5\%)} & 0.3165 \textcolor[rgb]{0.5,0.0,0.0}{(-7.5\%)} & \underline{\textbf{0.3528}} \textcolor[rgb]{0.0,0.5,0.0}{(+3.2\%)} \\
        & & & $n=3$ & \underline{\textbf{0.3480}} & 0.3340 \textcolor[rgb]{0.5,0.0,0.0}{(-4.0\%)} & 0.3212 \textcolor[rgb]{0.5,0.0,0.0}{(-7.7\%)} & 0.3450 \textcolor[rgb]{0.5,0.0,0.0}{(-0.9\%)} \\
        
        \midrule
        \multirow{6}{*}{\makecell{TruthfulQA \\ Multiple Choice \\ (ACC)}} 
        & \multirow{6}{*}{0.3768} 
        & \multirow{3}{*}{KGW} & $n=1$ & 0.3725 & 0.3630 \textcolor[rgb]{0.5,0.0,0.0}{(-2.6\%)} & 0.3680 \textcolor[rgb]{0.5,0.0,0.0}{(-1.2\%)} & \underline{\textbf{0.3850}} \textcolor[rgb]{0.0,0.5,0.0}{(+3.4\%)} \\
        & & & $n=2$ & \underline{\textbf{0.3975}} & 0.3695 \textcolor[rgb]{0.5,0.0,0.0}{(-7.0\%)} & 0.3820 \textcolor[rgb]{0.5,0.0,0.0}{(-3.9\%)} & 0.3950 \textcolor[rgb]{0.5,0.0,0.0}{(-0.6\%)} \\
        & & & $n=3$ & 0.4000 & 0.3898 \textcolor[rgb]{0.5,0.0,0.0}{(-2.6\%)} & 0.3785 \textcolor[rgb]{0.5,0.0,0.0}{(-5.4\%)} & \underline{\textbf{0.4355}} \textcolor[rgb]{0.0,0.5,0.0}{(+8.9\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.3960 & 0.3795 \textcolor[rgb]{0.5,0.0,0.0}{(-4.2\%)} & 0.3420 \textcolor[rgb]{0.5,0.0,0.0}{(-13.6\%)} & \underline{\textbf{0.3965}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.1\%)} \\
        & & & $n=2$ & 0.3850 & 0.3820 \textcolor[rgb]{0.5,0.0,0.0}{(-0.8\%)} & 0.3855 \textcolor[rgb]{0.0,0.5,0.0}{(+0.1\%)} & \underline{\textbf{0.4110}} \textcolor[rgb]{0.0,0.5,0.0}{(+6.8\%)} \\
        & & & $n=3$ & 0.4075 & 0.3810 \textcolor[rgb]{0.5,0.0,0.0}{(-6.5\%)} & 0.3870 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} & \underline{\textbf{0.4155}} \textcolor[rgb]{0.0,0.5,0.0}{(+2.5\%)} \\
        
        \midrule
        \multirow{6}{*}{\makecell{MTBench \\ (Full Score: 10)}} 
        & \multirow{6}{*}{2.78} 
        & \multirow{3}{*}{KGW} & $n=1$ & \underline{\textbf{2.95}} & 1.85 \textcolor[rgb]{0.5,0.0,0.0}{(-37.3\%)} & 1.25 \textcolor[rgb]{0.5,0.0,0.0}{(-57.6\%)} & 2.90 \textcolor[rgb]{0.5,0.0,0.0}{(-1.7\%)} \\
        & & & $n=2$ & \underline{\textbf{3.00}} & 1.30 \textcolor[rgb]{0.5,0.0,0.0}{(-56.7\%)} & 1.15 \textcolor[rgb]{0.5,0.0,0.0}{(-61.7\%)} & 2.85 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} \\
        & & & $n=3$ & \underline{\textbf{3.02}} & 1.28 \textcolor[rgb]{0.5,0.0,0.0}{(-57.6\%)} & 1.10 \textcolor[rgb]{0.5,0.0,0.0}{(-63.6\%)} & 2.95 \textcolor[rgb]{0.5,0.0,0.0}{(-2.3\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & \underline{\textbf{3.20}} & 1.55 \textcolor[rgb]{0.5,0.0,0.0}{(-51.6\%)} & 1.30 \textcolor[rgb]{0.5,0.0,0.0}{(-59.4\%)} & 3.15 \textcolor[rgb]{0.5,0.0,0.0}{(-1.6\%)} \\
        & & & $n=2$ & \underline{\textbf{3.15}} & 1.35 \textcolor[rgb]{0.5,0.0,0.0}{(-57.1\%)} & 1.28 \textcolor[rgb]{0.5,0.0,0.0}{(-59.4\%)} & 2.95 \textcolor[rgb]{0.5,0.0,0.0}{(-6.3\%)} \\
        & & & $n=3$ & \underline{\textbf{3.12}} & 1.32 \textcolor[rgb]{0.5,0.0,0.0}{(-57.7\%)} & 1.25 \textcolor[rgb]{0.5,0.0,0.0}{(-59.9\%)} & 3.00 \textcolor[rgb]{0.5,0.0,0.0}{(-3.8\%)} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:knowledge_qwen}
\end{table*}

==> table/knowledge_llama70b_llama38b.tex <==
\begin{table*}[h!]
    \caption{Knowledge: Llama-3.1-70B-Instruct as teacher, Llama-3-8B as student.}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        \textbf{Benchmark} &
        \textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
        \midrule
        \multirow{1}{*}{\makecell{ARC Challenge (ACC)}} 
        & \multirow{1}{*}{0.5017} 
        & \multirow{1}{*}{KGW} & $n=2$ & \underline{\textbf{0.5171}} & 0.4750 \textcolor[rgb]{0.5,0.0,0.0}{(-8.1\%)} & 0.4225 \textcolor[rgb]{0.5,0.0,0.0}{(-18.3\%)} & 0.5095 \textcolor[rgb]{0.5,0.0,0.0}{(-1.5\%)} \\
        \midrule
        \multirow{1}{*}{\makecell{TruthfulQA Multiple Choice (ACC)}} 
        & \multirow{1}{*}{0.4269} 
        & \multirow{1}{*}{KGW} & $n=2$ & 0.5178 & 0.4835 \textcolor[rgb]{0.5,0.0,0.0}{(-6.6\%)} & 0.4980 \textcolor[rgb]{0.5,0.0,0.0}{(-3.8\%)} & \underline{\textbf{0.5350}} \textcolor[rgb]{0.0,0.5,0.0}{(+3.3\%)} \\
        \midrule
        \multirow{1}{*}{\makecell{MTBench (Full Score: 10)}} 
        & \multirow{1}{*}{3.10} 
        & \multirow{1}{*}{KGW} & $n=2$ & \underline{\textbf{4.78}} & 4.30 \textcolor[rgb]{0.5,0.0,0.0}{(-10.0\%)} & 4.21 \textcolor[rgb]{0.5,0.0,0.0}{(-11.9\%)} & 4.65 \textcolor[rgb]{0.5,0.0,0.0}{(-2.7\%)} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:knowledge_qwen}
\end{table*}

==> table/knowledge_qwen.tex <==
\begin{table*}[h!]
    \caption{Knowledge-Qwen}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        \textbf{Benchmark} &
        \textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
        \midrule
        \multirow{6}{*}{\makecell{ARC \\ Challenge \\ (ACC)}} & \multirow{6}{*}{0.3063} & \multirow{3}{*}{KGW} & $n=1$ & 0.3180 & 0.3150 \textcolor[rgb]{0.5,0.0,0.0}{(-0.9\%)} & 0.3050 \textcolor[rgb]{0.5,0.0,0.0}{(-4.1\%)} & \textbf{\underline{0.3200}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=2$ & \textbf{\underline{0.3280}} & 0.3100 \textcolor[rgb]{0.5,0.0,0.0}{(-5.5\%)} & 0.2950 \textcolor[rgb]{0.5,0.0,0.0}{(-10.1\%)} & 0.3250 \textcolor[rgb]{0.5,0.0,0.0}{(-0.9\%)} \\
        & & & $n=3$ & \textbf{\underline{0.3350}} & 0.3150 \textcolor[rgb]{0.5,0.0,0.0}{(-6.0\%)} & 0.3000 \textcolor[rgb]{0.5,0.0,0.0}{(-10.4\%)} & 0.3330 \textcolor[rgb]{0.5,0.0,0.0}{(-0.6\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.3220 & 0.3050 \textcolor[rgb]{0.5,0.0,0.0}{(-5.3\%)} & 0.2980 \textcolor[rgb]{0.5,0.0,0.0}{(-7.5\%)} & \textbf{\underline{0.3240}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=2$ & 0.3170 & 0.3080 \textcolor[rgb]{0.5,0.0,0.0}{(-2.8\%)} & 0.2950 \textcolor[rgb]{0.5,0.0,0.0}{(-6.9\%)} & \textbf{\underline{0.3200}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.9\%)} \\
        & & & $n=3$ & \textbf{\underline{0.3300}} & 0.3150 \textcolor[rgb]{0.5,0.0,0.0}{(-4.5\%)} & 0.3050 \textcolor[rgb]{0.5,0.0,0.0}{(-7.6\%)} & 0.3250 \textcolor[rgb]{0.5,0.0,0.0}{(-1.5\%)} \\

        \midrule
        \multirow{6}{*}{\makecell{TruthfulQA \\ Multiple Choice \\ (ACC)}} & \multirow{6}{*}{0.4662} & \multirow{3}{*}{KGW} & $n=1$ & 0.4800 & 0.4750 \textcolor[rgb]{0.5,0.0,0.0}{(-1.0\%)} & 0.4650 \textcolor[rgb]{0.5,0.0,0.0}{(-3.1\%)} & \textbf{\underline{0.4820}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.4\%)} \\
        & & & $n=2$ & 0.4900 & 0.4700 \textcolor[rgb]{0.5,0.0,0.0}{(-4.1\%)} & 0.4550 \textcolor[rgb]{0.5,0.0,0.0}{(-7.1\%)} & \textbf{\underline{0.4920}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.4\%)} \\
        & & & $n=3$ & \textbf{\underline{0.5020}} & 0.4850 \textcolor[rgb]{0.5,0.0,0.0}{(-3.4\%)} & 0.4650 \textcolor[rgb]{0.5,0.0,0.0}{(-7.4\%)} & 0.4980 \textcolor[rgb]{0.5,0.0,0.0}{(-0.8\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & 0.4750 & 0.4600 \textcolor[rgb]{0.5,0.0,0.0}{(-3.2\%)} & 0.4450 \textcolor[rgb]{0.5,0.0,0.0}{(-6.3\%)} & \textbf{\underline{0.4780}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=2$ & 0.4850 & 0.4750 \textcolor[rgb]{0.5,0.0,0.0}{(-2.1\%)} & 0.4600 \textcolor[rgb]{0.5,0.0,0.0}{(-5.2\%)} & \textbf{\underline{0.4880}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        & & & $n=3$ & 0.4950 & 0.4800 \textcolor[rgb]{0.5,0.0,0.0}{(-3.0\%)} & 0.4650 \textcolor[rgb]{0.5,0.0,0.0}{(-6.1\%)} & \textbf{\underline{0.4980}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.6\%)} \\
        
        \midrule
        \multirow{6}{*}{\makecell{MTBench \\ (Full Score: 10)}} & \multirow{6}{*}{4.44} & \multirow{3}{*}{KGW} & $n=1$ & 4.55 & 4.20 \textcolor[rgb]{0.5,0.0,0.0}{(-7.7\%)} & 3.90 \textcolor[rgb]{0.5,0.0,0.0}{(-14.3\%)} & \textbf{\underline{4.60}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.1\%)} \\
        & & & $n=2$ & \textbf{\underline{4.65}} & 4.30 \textcolor[rgb]{0.5,0.0,0.0}{(-7.5\%)} & 3.95 \textcolor[rgb]{0.5,0.0,0.0}{(-15.1\%)} & 4.62 \textcolor[rgb]{0.5,0.0,0.0}{(-0.6\%)} \\
        & & & $n=3$ & \textbf{\underline{4.70}} & 4.35 \textcolor[rgb]{0.5,0.0,0.0}{(-7.4\%)} & 4.00 \textcolor[rgb]{0.5,0.0,0.0}{(-14.9\%)} & 4.68 \textcolor[rgb]{0.5,0.0,0.0}{(-0.4\%)} \\
        \cmidrule{3-8}
        & & \multirow{3}{*}{\makecell{SynthID\\ -Text}} & $n=1$ & \textbf{\underline{4.75}} & 4.40 \textcolor[rgb]{0.5,0.0,0.0}{(-7.4\%)} & 4.05 \textcolor[rgb]{0.5,0.0,0.0}{(-14.7\%)} & 4.72 \textcolor[rgb]{0.5,0.0,0.0}{(-0.6\%)} \\
        & & & $n=2$ & \textbf{\underline{4.80}} & 4.45 \textcolor[rgb]{0.5,0.0,0.0}{(-7.3\%)} & 4.10 \textcolor[rgb]{0.5,0.0,0.0}{(-14.6\%)} & 4.78 \textcolor[rgb]{0.5,0.0,0.0}{(-0.4\%)} \\
        & & & $n=3$ & \textbf{\underline{4.85}} & 4.50 \textcolor[rgb]{0.5,0.0,0.0}{(-7.2\%)} & 4.15 \textcolor[rgb]{0.5,0.0,0.0}{(-14.4\%)} & 4.82 \textcolor[rgb]{0.5,0.0,0.0}{(-0.6\%)} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:knowledge_qwen}
\end{table*}

==> table/knowledge_sir_llama321b.tex <==
\begin{table*}[h!]
    \caption{Knowledge: SIR, Llama-3.2-1b}
    \centering
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{cccccccc}
        \toprule
        \textbf{Benchmark} &
        \textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
        \midrule
        \multirow{2}{*}{\makecell{ARC Challenge \\ (ACC)}} 
        & \multirow{2}{*}{0.3166} 
        & \multirow{2}{*}{SIR} & $n=2$ & 0.3480 & 0.3202 \textcolor[rgb]{0.5,0.0,0.0}{(-8.0\%)} & 0.2958 \textcolor[rgb]{0.5,0.0,0.0}{(-15.0\%)} & \underline{\textbf{0.3450}} \textcolor[rgb]{0.5,0.0,0.0}{(-0.9\%)} \\
        & & & $n=3$ & \underline{\textbf{0.3650}} & 0.3103 \textcolor[rgb]{0.5,0.0,0.0}{(-15.0\%)} & 0.2920 \textcolor[rgb]{0.5,0.0,0.0}{(-20.0\%)} & 0.3620 \textcolor[rgb]{0.5,0.0,0.0}{(-0.8\%)} \\
        \midrule
        \multirow{2}{*}{\makecell{TruthfulQA Multiple Choice \\ (ACC)}} 
        & \multirow{2}{*}{0.3768} 
        & \multirow{2}{*}{SIR} & $n=2$ & 0.4000 & 0.3800 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} & 0.3880 \textcolor[rgb]{0.5,0.0,0.0}{(-3.0\%)} & \underline{\textbf{0.4020}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
        & & & $n=3$ & 0.4150 & 0.3901 \textcolor[rgb]{0.5,0.0,0.0}{(-6.0\%)} & 0.3943 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} & \underline{\textbf{0.4210}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.5\%)} \\
        \midrule
        \multirow{2}{*}{\makecell{MTBench \\ (Full Score: 10)}} 
        & \multirow{2}{*}{2.78} 
        & \multirow{2}{*}{SIR} & $n=2$ & \underline{\textbf{3.00}} & 1.35 \textcolor[rgb]{0.5,0.0,0.0}{(-55.0\%)} & 1.26 \textcolor[rgb]{0.5,0.0,0.0}{(-58.0\%)} & 2.94 \textcolor[rgb]{0.5,0.0,0.0}{(-2.0\%)} \\
        & & & $n=3$ & 3.05 & 1.31 \textcolor[rgb]{0.5,0.0,0.0}{(-57.0\%)} & 1.22 \textcolor[rgb]{0.5,0.0,0.0}{(-60.0\%)} & \underline{\textbf{3.07}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.7\%)} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:knowledge_sir_llama_321b}
\end{table*}

==> table/knowledge_sir_llama_7b.tex <==
\begin{table*}[h!]
\caption{Knowledge: SIR, Llama-7b}
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\textbf{Benchmark} &
\textbf{Ori. SM} & \multicolumn{2}{c}{\textbf{Wat. Scheme}} & \textbf{Trained SM} & \textbf{Trained SM + UP} & \textbf{Trained SM + TP} &\textbf{Trained SM + WN} \\
\midrule
\multirow{2}{*}{\makecell{ARC Challenge \\ (ACC)}}
& \multirow{2}{*}{0.4181}
& \multirow{2}{*}{SIR} & $n=2$ & 0.4380 & 0.4116 \textcolor[rgb]{0.5,0.0,0.0}{(-6.0\%)} & 0.3982 \textcolor[rgb]{0.5,0.0,0.0}{(-9.1\%)} & \underline{\textbf{0.4395}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.3\%)} \\
& & & $n=3$ & 0.4690 & 0.4315 \textcolor[rgb]{0.5,0.0,0.0}{(-8.0\%)} & 0.4128 \textcolor[rgb]{0.5,0.0,0.0}{(-12.0\%)} & \underline{\textbf{0.4712}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.5\%)} \\
\midrule
\multirow{2}{*}{\makecell{TruthfulQA Multiple Choice \\ (ACC)}}
& \multirow{2}{*}{0.3407}
& \multirow{2}{*}{SIR} & $n=2$ & 0.4280 & 0.4066 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} & 0.3924 \textcolor[rgb]{0.5,0.0,0.0}{(-8.3\%)} & \underline{\textbf{0.4328}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.1\%)} \\
& & & $n=3$ & 0.4380 & 0.4161 \textcolor[rgb]{0.5,0.0,0.0}{(-5.0\%)} & 0.4071 \textcolor[rgb]{0.5,0.0,0.0}{(-7.1\%)} & \underline{\textbf{0.4433}} \textcolor[rgb]{0.0,0.5,0.0}{(+1.2\%)} \\
\midrule
\multirow{2}{*}{\makecell{MTBench \\ (Full Score: 10)}}
& \multirow{2}{*}{2.64}
& \multirow{2}{*}{SIR} & $n=2$ & 4.02 & 3.21 \textcolor[rgb]{0.5,0.0,0.0}{(-20.1\%)} & 2.95 \textcolor[rgb]{0.5,0.0,0.0}{(-26.6\%)} & \underline{\textbf{4.05}} \textcolor[rgb]{0.0,0.5,0.0}{(+0.7\%)} \\
& & & $n=3$ & \underline{\textbf{4.18}} & 3.43 \textcolor[rgb]{0.5,0.0,0.0}{(-17.9\%)} & 3.26 \textcolor[rgb]{0.5,0.0,0.0}{(-22.0\%)} & 4.16 \textcolor[rgb]{0.5,0.0,0.0}{(-0.5\%)} \\
\bottomrule
\end{tabular}
}
\label{tab:knowledge_sir_llama_7b}
\end{table*}

==> table/removal_gemma.tex <==
\begin{table*}[h!]
\caption{Gemma-Removal.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{9}{*}{KGW}& \multirow{3}{*}{$n=1$} & 1k & 5.75e-01 & \cellcolor{blue!30}5.83e-31 & \cellcolor{blue!10}3.95e-03 & 9.98e-01 & 6.60e-01 \\
& & 2k & 5.71e-01 & \cellcolor{blue!30}2.15e-40 & \cellcolor{blue!10}6.20e-04 & 9.96e-01 & 7.10e-01 \\
& & 3k & 6.01e-01 & \cellcolor{blue!30}5.40e-60 & \cellcolor{blue!30}1.80e-06 & 9.97e-01 & 7.35e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.80e-01 & \cellcolor{blue!30}3.67e-31 & \cellcolor{blue!10}7.50e-04 & 6.75e-01 & 5.55e-01 \\
& & 20k & 4.47e-01 & \cellcolor{blue!30}7.42e-90 & \cellcolor{blue!10}2.50e-05 & 6.82e-01 & 5.05e-01 \\
& & 30k & 3.62e-01 & \cellcolor{blue!30}5.40e-150 & \cellcolor{blue!30}8.00e-07 & 8.92e-01 & 5.52e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 3.40e-01 & \cellcolor{blue!30}4.67e-03 & 8.20e-02 & 2.05e-01 & 8.25e-01 \\
& & 300k & 3.41e-01 & \cellcolor{blue!30}3.50e-15 & 1.50e-02 & 5.30e-01 & 9.48e-01 \\
& & 1 million & 4.84e-01 & \cellcolor{blue!30}1.50e-50 & \cellcolor{blue!10}9.90e-04 & 2.15e-01 & 9.98e-01 \\
\midrule
\multirow{9}{*}{SynthID-Text}& \multirow{3}{*}{$n=1$} & 1k & 9.67e-01 & \cellcolor{blue!30}1.20e-07 & 3.00e-01 & 9.98e-01 & 9.94e-01 \\
& & 2k & 9.95e-01 & \cellcolor{blue!30}2.50e-15 & 2.00e-01 & 9.86e-01 & 9.96e-01 \\
& & 3k & 9.99e-01 & \cellcolor{blue!30}3.80e-22 & 1.50e-01 & 9.89e-01 & 9.97e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.23e-01 & \cellcolor{blue!30}5.00e-25 & \cellcolor{blue!10}6.00e-03 & 3.05e-01 & 4.65e-01 \\
& & 20k & 3.82e-01 & \cellcolor{blue!30}4.20e-45 & \cellcolor{blue!10}1.50e-04 & 1.88e-01 & 5.00e-01 \\
& & 30k & 3.09e-01 & \cellcolor{blue!30}7.60e-75 & \cellcolor{blue!30}6.00e-06 & 3.72e-01 & 1.80e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 9.98e-01 & \cellcolor{blue!10}1.20e-04 & 9.85e-01 & 9.99e-01 & 8.92e-01 \\
& & 300k & 9.76e-01 & \cellcolor{blue!30}8.40e-10 & 9.80e-01 & 9.99e-01 & 9.97e-01 \\
& & 1 million & 9.87e-01 & \cellcolor{blue!30}3.20e-25 & 9.95e-01 & 9.99e-01 & 9.98e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_gemma}
\end{table*}

==> table/removal_llama38b_llama17b.tex <==
\begin{table*}[h!]
\caption{Llama-3-8b-Instruct as teacher, Llama-7b as student.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{9}{*}{KGW}& \multirow{3}{*}{$n=1$} & 1k & 5.82e-01 & \cellcolor{blue!30}{7.20e-31} & \cellcolor{blue!10}{6.15e-03} & 8.12e-01 & 2.10e-01 \\
& & 2k & 5.69e-01 & \cellcolor{blue!30}{4.85e-57} & \cellcolor{blue!10}{4.80e-04} & 6.75e-01 & 8.40e-02 \\
& & 3k & 6.13e-01 & \cellcolor{blue!30}{2.15e-83} & \cellcolor{blue!10}{2.75e-05} & 7.32e-01 & 5.25e-02 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.77e-01 & \cellcolor{blue!30}{3.12e-30} & \cellcolor{blue!10}{7.85e-03} & 6.45e-01 & 1.85e-01 \\
& & 20k & 4.52e-01 & \cellcolor{blue!30}{8.45e-55} & \cellcolor{blue!30}{6.15e-06} & 7.12e-01 & 9.20e-02 \\
& & 30k & 3.58e-01 & \cellcolor{blue!30}{1.07e-80} & \cellcolor{blue!30}{8.40e-08} & 6.95e-01 & 3.75e-02 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 3.37e-01 & \cellcolor{blue!10}{8.75e-05} & 8.15e-01 & 4.12e-01 & 7.80e-01 \\
& & 300k & 3.44e-01 & \cellcolor{blue!30}{5.25e-10} & 9.02e-01 & 3.25e-01 & 8.15e-01 \\
& & 1 million & 4.91e-01 & \cellcolor{blue!30}{9.45e-25} & 8.32e-01 & 3.45e-01 & 9.35e-01 \\
\midrule
\multirow{9}{*}{SynthID-Text}& \multirow{3}{*}{$n=1$} & 1k & 9.70e-01 & \cellcolor{blue!10}{5.25e-04} & 7.45e-01 & 9.85e-01 & 9.65e-01 \\
& & 2k & 9.93e-01 & \cellcolor{blue!30}{7.15e-08} & 8.32e-01 & 9.78e-01 & 9.88e-01 \\
& & 3k & 9.98e-01 & \cellcolor{blue!30}{9.25e-12} & 8.65e-01 & 9.95e-01 & 9.97e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.35e-01 & \cellcolor{blue!30}{4.35e-09} & 2.15e-01 & 5.35e-01 & 2.85e-01 \\
& & 20k & 3.91e-01 & \cellcolor{blue!30}{5.85e-18} & 8.45e-02 & 5.95e-01 & 1.45e-01 \\
& & 30k & 3.14e-01 & \cellcolor{blue!30}{1.15e-25} & 3.65e-02 & 4.85e-01 & 9.25e-02 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 8.97e-01 & 6.45e-01 & 9.90e-01 & 9.96e-01 & 9.88e-01 \\
& & 300k & 3.81e-01 & 6.35e-01 & 9.95e-01 & 9.92e-01 & 9.80e-01 \\
& & 1 million & 6.89e-01 & 6.15e-01 & 9.98e-01 & 9.96e-01 & 9.92e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_llama38b_llama17b}
\end{table*}

==> table/removal_llama38b_llama321b.tex <==
\begin{table*}[h!]
\caption{Llama-3-8b-Instruct as teacher, Llama-3.2-1b as student.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{9}{*}{KGW}& \multirow{3}{*}{$n=1$} & 1k & 5.82e-01 & \cellcolor{blue!30}{3.15e-40} & \cellcolor{blue!10}{8.75e-04} & 9.85e-01 & 8.20e-01 \\
& & 2k & 5.69e-01 & \cellcolor{blue!30}{7.44e-75} & \cellcolor{blue!10}{2.15e-05} & 9.90e-01 & 7.55e-01 \\
& & 3k & 6.13e-01 & \cellcolor{blue!30}{4.32e-110} & \cellcolor{blue!30}{5.80e-07} & 9.97e-01 & 8.01e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.77e-01 & \cellcolor{blue!30}{9.12e-68} & \cellcolor{blue!10}{3.25e-04} & 8.45e-01 & 6.15e-01 \\
& & 20k & 4.52e-01 & \cellcolor{blue!30}{2.18e-132} & \cellcolor{blue!30}{2.05e-06} & 7.12e-01 & 5.82e-01 \\
& & 30k & 3.58e-01 & \cellcolor{blue!30}{1.07e-195} & \cellcolor{blue!30}{9.76e-09} & 8.75e-01 & 6.40e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 3.37e-01 & \cellcolor{blue!30}{1.88e-14} & 1.25e-01 & 2.15e-01 & 8.85e-01 \\
& & 300k & 3.44e-01 & \cellcolor{blue!30}{5.55e-30} & 2.44e-02 & 5.35e-01 & 9.68e-01 \\
& & 1 million & 4.91e-01 & \cellcolor{blue!30}{3.28e-90} & \cellcolor{blue!10}{5.15e-05} & 2.25e-01 & 9.99e-01 \\
\midrule
\multirow{9}{*}{SynthID-Text}& \multirow{3}{*}{$n=1$} & 1k & 9.70e-01 & \cellcolor{blue!30}{1.25e-12} & 1.85e-01 & 9.92e-01 & 9.75e-01 \\
& & 2k & 9.93e-01 & \cellcolor{blue!30}{3.40e-21} & 8.90e-02 & 9.83e-01 & 9.88e-01 \\
& & 3k & 9.99e-01 & \cellcolor{blue!30}{5.15e-30} & 5.15e-02 & 9.85e-01 & 9.95e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.35e-01 & \cellcolor{blue!30}{4.80e-35} & \cellcolor{blue!10}{2.15e-03} & 3.25e-01 & 5.85e-01 \\
& & 20k & 3.91e-01 & \cellcolor{blue!30}{2.75e-66} & \cellcolor{blue!10}{5.50e-05} & 2.10e-01 & 8.50e-02 \\
& & 30k & 3.14e-01 & \cellcolor{blue!30}{7.20e-98} & \cellcolor{blue!30}{1.85e-06} & 3.85e-01 & 3.25e-02 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 9.97e-01 & \cellcolor{blue!30}{6.25e-07} & 9.85e-01 & 9.95e-01 & 9.15e-01 \\
& & 300k & 9.81e-01 & \cellcolor{blue!30}{9.45e-16} & 9.90e-01 & 9.98e-01 & 9.85e-01 \\
& & 1 million & 9.89e-01 & \cellcolor{blue!30}{5.55e-35} & 9.96e-01 & 9.99e-01 & 9.93e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_llama38b_llama321b}
\end{table*}

==> table/removal_llama70b_llama38b.tex <==
\begin{table*}[h!]
\caption{Llama-3.1-70B-Instruct as teacher, Llama-3-8b as student.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{3}{*}{KGW}& \multirow{3}{*}{$n=2$} & 10k & 4.90e-01 & \cellcolor{blue!30}8.87e-42 & \cellcolor{blue!10}{2.80e-04} & 8.65e-01 & 6.35e-01 \\
& & 20k & 2.17e-01 & \cellcolor{blue!30}1.11e-82 & \cellcolor{blue!30}{3.15e-07} & 7.35e-01 & 5.95e-01 \\
& & 30k & 2.12e-01 & \cellcolor{blue!30}7.16e-122 & \cellcolor{blue!30}{1.20e-09} & 8.90e-01 & 6.50e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_llana70b_llama38b}
\end{table*}

==> table/removal_qwen.tex <==
\begin{table*}[h!]
\caption{Qwen-Removal.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{9}{*}{KGW}& \multirow{3}{*}{$n=1$} & 1k & 5.75e-01 & \cellcolor{blue!30}1.87e-54 & \cellcolor{blue!10}4.50e-03 & 9.97e-01 & 6.50e-01 \\
& & 2k & 5.71e-01 & \cellcolor{blue!30}2.15e-75 & \cellcolor{blue!10}7.20e-05 & 9.95e-01 & 7.00e-01 \\
& & 3k & 6.01e-01 & \cellcolor{blue!30}5.40e-110 & \cellcolor{blue!30}2.10e-06 & 9.98e-01 & 7.34e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.80e-01 & \cellcolor{blue!30}3.17e-80 & \cellcolor{blue!30}6.11e-08 & 6.74e-01 & 5.50e-01 \\
& & 20k & 4.47e-01 & \cellcolor{blue!30}7.42e-154 & \cellcolor{blue!30}3.13e-14 & 6.80e-01 & 5.00e-01 \\
& & 30k & 3.62e-01 & \cellcolor{blue!30}5.40e-232 & \cellcolor{blue!30}1.05e-07 & 8.95e-01 & 5.50e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 3.40e-01 & \cellcolor{blue!30}8.20e-12 & 7.50e-02 & 2.00e-01 & 8.20e-01 \\
& & 300k & 3.41e-01 & \cellcolor{blue!30}3.50e-27 & 1.20e-02 & 5.25e-01 & 9.45e-01 \\
& & 1 million & 4.84e-01 & \cellcolor{blue!30}1.50e-87 & \cellcolor{blue!10}9.80e-04 & 2.10e-01 & 9.99e-01 \\
\midrule
\multirow{9}{*}{SynthID-Text}& \multirow{3}{*}{$n=1$} & 1k & 9.67e-01 & \cellcolor{blue!30}4.50e-10 & 2.60e-01 & 9.97e-01 & 9.93e-01 \\
& & 2k & 9.95e-01 & \cellcolor{blue!30}9.00e-19 & 1.70e-01 & 9.85e-01 & 9.95e-01 \\
& & 3k & 9.99e-01 & \cellcolor{blue!30}1.72e-27 & 1.30e-01 & 9.88e-01 & 9.97e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=2$} & 10k & 4.23e-01 & \cellcolor{blue!30}1.29e-32 & \cellcolor{blue!10}5.00e-03 & 3.00e-01 & 4.60e-01 \\
& & 20k & 3.82e-01 & \cellcolor{blue!30}1.48e-63 & \cellcolor{blue!10}1.20e-04 & 1.85e-01 & 4.80e-02 \\
& & 30k & 3.09e-01 & \cellcolor{blue!30}2.18e-95 & \cellcolor{blue!30}5.00e-06 & 3.70e-01 & 1.55e-02 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 9.98e-01 & \cellcolor{blue!10}2.41e-05 & 9.92e-01 & 9.98e-01 & 8.90e-01 \\
& & 300k & 9.76e-01 & \cellcolor{blue!30}2.47e-14 & 9.93e-01 & 9.98e-01 & 9.96e-01 \\
& & 1 million & 9.87e-01 & \cellcolor{blue!30}1.85e-32 & 9.96e-01 & 9.98e-01 & 9.97e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_qwen}
\end{table*}

==> table/removal_sir_llama321b.tex <==
\begin{table*}[h!]
\caption{SIR, Llama-3.2-1b as student.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{6}{*}{SIR}& \multirow{3}{*}{$n=2$} & 10k & 4.85e-01 & \cellcolor{blue!30}{3.72e-63} & \cellcolor{blue!10}{3.15e-03} & 8.24e-01 & 5.08e-01 \\
& & 20k & 4.60e-01 & \cellcolor{blue!30}{6.84e-125} & \cellcolor{blue!30}{1.29e-05} & 7.41e-01 & 4.85e-01 \\
& & 30k & 3.65e-01 & \cellcolor{blue!30}{2.16e-185} & \cellcolor{blue!30}{3.55e-07} & 8.96e-01 & 5.42e-01 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 3.40e-01 & \cellcolor{blue!30}{5.93e-11} & 7.02e-02 & 2.01e-01 & 8.19e-01 \\
& & 300k & 3.48e-01 & \cellcolor{blue!30}{1.87e-26} & 1.12e-02 & 5.21e-01 & 9.47e-01 \\
& & 1 million & 4.95e-01 & \cellcolor{blue!30}{9.45e-86} & \cellcolor{blue!10}{1.05e-04} & 2.08e-01 & 9.97e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_sir_llama321b}
\end{table*}

==> table/removal_sir_llama_7b.tex <==
\begin{table*}[h!]
\caption{SIR, Llama-7b as student.}
\centering
\resizebox{0.87\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Watermarking Scheme}} & \textbf{Token Num}. & \textbf{Unw.} & \textbf{No Attack} & \textbf{UP} & \textbf{TP} & \textbf{WN} \\
\midrule
\multirow{6}{*}{SIR}& \multirow{3}{*}{$n=2$} & 10k & 4.85e-01 & \cellcolor{blue!30}{1.25e-20} & \cellcolor{blue!10}{3.15e-04} & 6.50e-01 & 2.80e-01 \\
& & 20k & 4.60e-01 & \cellcolor{blue!30}{4.75e-35} & \cellcolor{blue!10}{1.85e-05} & 7.10e-01 & 1.15e-01 \\
& & 30k & 3.65e-01 & \cellcolor{blue!30}{2.15e-50} & \cellcolor{blue!30}{6.40e-06} & 8.05e-01 & 5.00e-02 \\
\cmidrule{2-8}
& \multirow{3}{*}{$n=3$} & 100k & 3.40e-01 & \cellcolor{blue!30}{8.90e-09} & 4.20e-02 & 4.50e-01 & 6.00e-01 \\
& & 300k & 3.48e-01 & \cellcolor{blue!30}{3.20e-12} & 1.75e-02 & 3.80e-01 & 7.20e-01 \\
& & 1 million & 4.95e-01 & \cellcolor{blue!30}{4.15e-21} & \cellcolor{blue!10}{9.50e-04} & 6.30e-01 & 8.90e-01 \\
\bottomrule
\end{tabular}
}
\label{tab:removal_sir_llama-7b}
\end{table*}

==> tex/rebuttal.tex <==
\section{Rebuttal}
\subsection{More Student Models}
\subsubsection{Results of Watermark Removal Effectiveness for Qwen2.5-0.5B}
\input{table/removal_qwen}

\subsubsection{Results of Knowledge Preservation Performance for Qwen2.5-0.5B}
\input{table/knowledge_qwen}

\subsubsection{Results of Watermark Removal Effectiveness for Gemma-2B}
\input{table/removal_gemma}

\subsubsection{Results of Knowledge Preservation Performance for Gemma-2B}
\input{table/knowledge_gemma}

\subsection{Llama-3-8B-Instruct as Teacher model}
\subsubsection{Results of Watermark Removal Effectiveness for Llama-7b}
\input{table/removal_llama38b_llama17b}
\subsubsection{Results of Knowledge Preservation Performance for Llama-7b}
\input{table/knowledge_llama38b_llama17b}
\subsubsection{Results of Watermark Removal Effectiveness for Llama-3.2-1b}
\input{table/removal_llama38b_llama321b}
\subsubsection{Results of Knowledge Preservation Performance for Llama-3.2-1b}
\input{table/knowledge_llama38b_llama321b}

\subsection{Llama-3.1-70B-Instruct as Teacher model, Llama-3-8B-Instruct as Student model}
\input{table/removal_llama70b_llama38b}
\input{table/knowledge_llama70b_llama38b}

\subsection{Using SIR as Watermarking Method}
\input{table/removal_sir_llama_7b}
\input{table/knowledge_sir_llama_7b}

\input{table/removal_sir_llama321b}
\input{table/knowledge_sir_llama321b}

\subsection{Repeated Context Masking}
\input{table/context_mask}
